Galaxy Rotation Curves from String Theory

This is a speculative attempt to connect string theory with cosmological observation. Inspired by an exactly solvable model in string theory, and based on the assumption that all matter is made of strings, individual stars will couple universally to this string gauge field and execute Landau orbits, much like electrons in an external magnetic field. This three-parameter phenomenological model can adequately fit the galaxy rotation curves. The extra centripetal acceleration provided by the background field can hence account for the "missing mass" needed to sustain the high rotation speed beyond the bulk of the stellar mass. The rotation speed of the stars on the outskirts of a galaxy is predicted to be linearly rising with distance.

==> mass_table.tex <==
\\ \hlline
galaxy&   likelihood&   ½&   ?&   Rd (kpc)&   total mass(Msun)&   B magnitude&   mass/light \\ \hline
\\ \hline
 ngc0628&   4.35&   8.872&   11738&   1.803&   3.35E+10&   -20.60&   1.24\\ \hline   
 ngc0925&   2.45&   5.077&   500&   2.473&   3.68E+09&   -20.05&   0.23\\ \hline   
 ngc2403&   4.25&   13.418&   16497&   0.518&   1.12E+09&   -19.56&   0.11\\ \hline   
 ngc2976&   0.40&   0.100&   2135&   1.867&   6.76E+09&   -18.12&   2.45\\ \hline   
 ngc3031&   5.70&   2.000&   3187&   4.389&   1.31E+11&   -21.54&   2.04\\ \hline   
 ngc3184&   0.57&   0.655&   1552&   4.685&   7.77E+10&   -19.88&   5.58\\ \hline   
 ngc3198&   0.27&   1.968&   1971&   3.522&   4.19E+10&   -20.44&   1.80\\ \hline   
 ngc3521&   0.59&   6.046&   26678&   1.479&   4.20E+10&   -21.08&   1.00\\ \hline   
 ngc3621&   0.37&   10.338&   7413&   1.084&   4.60E+09&   -20.51&   0.18\\ \hline   
 ngc3938&   1.03&   9.722&   16199&   1.240&   1.50E+10&   -20.01&   0.96\\ \hline   
 ngc4236&   0.33&   10.358&   110&   2.022&   4.42E+08&   -18.10&   0.16\\ \hline   
 ngc4321&   2.07&   5.208&   3752&   3.148&   5.70E+10&   -22.06&   0.55\\ \hline   
 ngc4536&   0.74&   1.465&   734&   5.867&   7.22E+10&   -21.79&   0.89\\ \hline   
 ngc4569&   0.66&   16.370&   12262&   1.042&   6.75E+09&   -21.10&   0.16\\ \hline   
 ngc4579&   0.69&   7.385&   5164&   3.000&   6.79E+10&   -21.68&   0.93\\ \hline   
 ngc4625&   0.55&   0.100&   1140&   1.446&   1.68E+09&   -17.63&   0.96\\ \hline   
 ngc4725&   0.27&   1.378&   1523&   6.726&   2.26E+11&   -21.76&   2.87\\ \hline   
 ngc5055&   3.52&   4.064&   24581&   1.544&   4.40E+10&   -21.20&   0.94\\ \hline   
 ngc5194&   0.81&   3.186&   10718&   1.102&   6.98E+09&   -20.51&   0.28\\ \hline   
 ngc6946&   6.03&   7.440&   4980&   1.805&   1.43E+10&   -20.89&   0.40\\ \hline   
 ngc7331&   0.52&   8.465&   18613&   1.680&   4.30E+10&   -21.58&   0.64\\ \hline  
  m81dwb&   0.13&   1.119&   15919&   0.147&   2.46E+07&   -12.5&   1.58\\ \hline 
 <chi>&   1.65&   &   &   &   &   &   \\ \hline
